Exploring the mysterious high-ionization source powering [Ne V] in high-z analog SBS0335-052 E with JWST/MIRI

Nearby blue compact dwarf galaxies (BCDs) share similar properties with objects from the Epoch of Reionization revealed by JWST, in terms of low stellar mass, low metallicity and high specific star-formation rate. Thus, they represent ideal local laboratories for detailed multi-wavelength studies to understand their properties and the mechanisms shaping them. We report the first JWST MIRI/MRS observations of the BCD SBS 0335-052 E, analyzing MIR emission lines tracing different levels of ionization (e.g., [NeII], [SIV], [NeIII], [OIV], [NeV]) of the ionized gas. SBS 0335-052 E MIR emission is characterized by a bright point source, located in one of the youngest and most embedded stellar clusters ($t\sim3$ Myr, $A_V\sim15$), and underlying extended high-ionization emission (i.e., [OIV], [NeV]) from the surroundings of the older and less dusty stellar clusters ($t< 20 $ Myr, $A_V\sim8$). From the comparison with state-of-the-art models, we can exclude shocks, X-ray binaries, and old stellar populations as the main sources of the high ionization. Interestingly, a 4-16% contribution of a $\sim10^5$ M$_\odot$ intermediate massive black hole (IMBH) is needed to justify the strong [NeV]/[NeII] and would be consistent with optical/UV line ratios from previous studies. However, even IMBH models cannot explain the strongest [OIV]/[NeIII]. Also, star-forming models (regardless of including X-ray binaries) struggle to reproduce even the lower ionization line ratios (e.g., [SIV]/[NeII]) typically observed in BCDs. Overall, while current models suggest the need to account for an accreting IMBH in this high-$z$ analog, limitations still exist in predicting high-ionization emission lines (I.P. $>54$ eV) when modeling these low-metallicity environments, thus other sources of ionization cannot be fully ruled out.

==> Table2_orig.tex <==
 \begin{tabular}{lccccc} 
            Region & Age [Myr]    & Mass [$M_\odot$]                    & 12+log(O/H)                & \multicolumn{2}{c}{Other features}  \\
        \hline 
        SSC1   & 3.0 &  4.7$\times 10^5$ & \multirow{2}{*}{7.31}         &                   \multicolumn{2}{c}{Point source in MIRI-MRS and NICMOS 1.6~$\mu$m (T09)} \\ %\hline
        SSC2   & 3.0 &  3.7$\times 10^5$ &                               &     \multicolumn{2}{c}{SSC1-2 uniquely has dust and H$_2$, and thermal radio emission (J09)} \\ %\hline 
        SSC3   & 7.0   &  7.1$\times 10^5$ &       7.31             &  \multicolumn{2}{c}{WR Blue bump (P06; K18)} \\ 
        SSC4   & 11.0  &  1.1$\times 10^6$ & \multirow{2}{*}{7.27}  &  \multicolumn{2}{c}{SSCs4-5 characterized by $\sigma$(\nev) peak and tentative radio emission (J09)} \\ %\hline
        SSC5   & 13.0  &  2.9$\times 10^6$ &                               & \multicolumn{2}{c}{Point source in NICMOS 1.6~$\mu$m (T09)} \\ %\hline
        SSC6   & 11.0  &  2.6$\times 10^5$ &           ---                    & \multicolumn{2}{c}{Point source in NICMOS 1.6~$\mu$m (T09); $\sigma$(\siv) and  $\sigma$(\neiii) peak} \\ %\hline
        S3-Pa$\alpha$&  $<3$(?)    &          ---         &          7.38                     &  Bright H lines (T09) \\ %\hline
        S7     &    $<3$(?)        &          ---         &         7.10                      & \multicolumn{2}{c}{Bright H lines (T09); \nev/\neii\ and \oiv/\neiii\ peak} \\ 
        S8     &     ---       &          ---         &        7.21            & $\times$                            & \\ %\hline
        ULX    &      ---      &       ---            &         ---                      & \multicolumn{2}{c}{Revealed by P13 (see also K18))} \\ %\hline
        \hline
         % & \multicolumn{4}{c}{Line ratios} \\ 
        Region &log(\neiii/\neii) & log(\nev/\neii) & log(\oiv/\neiii) & log(\siv/\neii) & \nev~$\lambda$14.3$\mu$m           \\
        \hline
        SSC1               & $1.34\pm0.03$  & $<-0.53$  & $-0.40\pm0.07$  & $1.71\pm0.03$ &  $\times$  \\ %\hline
        SSC2               & $-0.13\pm0.01$ & ---  & $-0.7\pm0.5$ & $0.546\pm0.004$ & $\times$  \\ %\hline
        SSC3+S3-Pa$\alpha$ & $1.36\pm0.01$  & $-0.14\pm0.02$ & $-0.29\pm0.01$ & $1.64\pm0.01$ &  \checkmark \\ %\hline
        SSC4-5             & $1.19\pm0.04$  & $0.16\pm0.04$  & $0.05\pm0.01$ & $1.64\pm0.03$ & \checkmark \\ %\hline
        SSC6               & $0.85\pm0.04$  & $-0.20\pm0.04$ & $-0.07\pm0.02$ & $1.18\pm0.03$ & \checkmark \\ %\hline
        S7                 & $1.31\pm0.02$  & $0.35\pm0.02$  & $0.11\pm0.01$ & $1.66\pm0.02$ & \checkmark \\ %\hline
        S8                 & $0.60\pm0.08$  & ---   & --- & $1.08\pm0.04$ & $\times$     \\ %\hline
        ULX                & $1.11\pm0.02$ & $-0.43\pm0.04$ & $0.48\pm0.02$ & $1.14\pm0.02$ &\checkmark \\ %\hline
        \hline
         % & \multicolumn{4}{c}{Modelling} \\ 
        Region & \multicolumn{5}{c}{Modeling} \\ %SSP model & SXP & R22 & Shocks & Comments\\
        \\\hline
        SSC1   & \multicolumn{5}{c}{\citetalias{martinez-paredes2023} 2.5~Myr SSP with $M_{up}=300$~M$_\odot$ good for MIR line ratios but \siv/\neii; \citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs overpredict \nev\ upper limit} \\ %\hline
        SSC2   & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs reproduce \neiii/\neii\ vs \siv/\neii} \\ %\hline
        SSC3+S3-Pa$\alpha$   & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs reproduce \neiii/\neii\ vs \siv/\neii}\\ %\hline
        SSC4+5   & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs with ... }\\ %\hline
        SSC6   & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs with ... }\\ %\hline
        S7     & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs with ... }\\ %\hline
        S8     & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs reproduce \neiii/\neii\ vs \siv/\neii}\\ %\hline
        ULX    & \multicolumn{5}{c}{\citetalias{richardson2022} $M_{BH}=10^5$~M$_\odot$ IMBHs with ... } \\ %\hline
    \end{tabular}
